Observation of a Narrow Near-Threshold Structure in the $J/\psi\phi$ Mass Spectrum in $B^+\to J/\psi\phi K^+$ Decays

Observation is reported for a structure near the $J/\psi\phi$ threshold in $B^+\rightarrow J/\psi\phi K^+$ decays produced in $\bar{p} p $ collisions at $\sqrt{s}=1.96 \TeV$ with a statistical significance of beyond 5 standard deviations.

==> abstract.tex <==
Observation is reported for a structure  near  the  $J/\psi\phi$ threshold  
in  $B^+\rightarrow J/\psi\phi K^+$ decays produced in $\bar{p} p $
collisions at $\sqrt{s}=1.96~\TeV$  with a statistical significance of   
beyond 5 standard deviations. 

